Mining for Species, Locations, Habitats, and Ecosystems from Scientific Papers in Invasion Biology: A Large-Scale Exploratory Study with Large Language Models

This paper presents an exploratory study that harnesses the capabilities of large language models (LLMs) to mine key ecological entities from invasion biology literature. Specifically, we focus on extracting species names, their locations, associated habitats, and ecosystems, information that is critical for understanding species spread, predicting future invasions, and informing conservation efforts. Traditional text mining approaches often struggle with the complexity of ecological terminology and the subtle linguistic patterns found in these texts. By applying general-purpose LLMs without domain-specific fine-tuning, we uncover both the promise and limitations of using these models for ecological entity extraction. In doing so, this study lays the groundwork for more advanced, automated knowledge extraction tools that can aid researchers and practitioners in understanding and managing biological invasions.

==> sections/intro_sina.tex <==

Human population growth and expansion are coupled with the intentional and unintentional movement of species beyond their historic ranges. 
The introduction of nonnative species can have dramatic impacts that cascade across ecological scales from individual plants and animals to populations and communities \cite{roy2023ipbes}. 
The goal of invasion biology is to identify and understand the impacts of alien species on native flora and fauna across these ecological scales, not only to conserve rare, sensitive, and ecologically valuable native species, but also because intact functional ecosystems provide important economic, public health, and socioemotional services to humans \cite{cassey2018invasion,jeschke2018invasion}. 
Achieving this goal becomes increasingly challenging though, since alien species introductions operate at a rapid rate and global scale, and in the context of increasing human population growth and climate change.
Additionally, the body of research in this domain of ecology is currently growing to an extent that it becomes more and more difficult for invasion biology researchers to build a systematic and shared understanding of the impacts of alien species on ecosystems, or to even comprehensively categorize these species, and their locations, and relationships. This paper explores the potential of recent NLP technologies, such as Information Extraction (IE) approaches based on Large Language Models (LLMs), as a tool that could contribute to predicting future invasions and their consequences.

The extraction and categorization of information from scientific studies and publications is a well-known NLP task \cite{augenstein-etal-2017-semeval,gabor-etal-2018-semeval}. 
In the biomedical domain, NER and RE facilitate large-scale biomedical data analysis, such as network biology \cite{biomed1}, gene prioritization \cite{biomed2}, drug repositioning \cite{biomed3} and the creation of curated databases \cite{biomed4}. 
In the clinical domain, NER and RE can aid in disease and treatment prediction, readmission prediction, deidentification, and patient cohort identification \cite{miotto2018deep}.
However, the domain of ecology and invasion biology in particular has hardly been explored and dedicated datasets are scarce.
%In the domain of biodiversity, Named Entity Reccognition datasets exist that focus on tagging species \cite{gerner2010linnaeus,pafilis2013species}, specific concepts like bacteria and their locations \cite{deleger2016overview}, or combinations of species, habitats, locations \cite{nguyen2019copious}. \citet{loffler-etal-2020-tag} present the QEMP benchmark, which further extends the types of entities and links them to existing ontologies in biodiversity research. 
To the best of our knowledge, the small-scale INAS dataset \citep{brinner-etal-2022-linking} presents the only invasion biology-specific resource that  provides annotations of hypotheses for scientific abstracts.

This paper presents a study on information extraction (IE) in invasion biology, encompassing both named entity recognition (NER) and relation extraction (RE). We simultaneously build on studies showing that jointly learning NER and RE can enhance overall performance \cite{giorgi2019end} and on recent large language models (LLMs) which may open new opportunities for IE. 
Thus, our central question is whether LLMs, with their advanced pattern recognition capabilities, can be effectively applied to a new domain to simultaneously identify entities and infer their relationships.
We present an approach that prompts LLMs to identify the following four key entities in invasion biology--viz. species, location, habitat, and ecosystem. Since we cannot evaluate the results quantitatively, we explore them qualitatively with respect to the following questions: (i) do the LLMs extract reasonable species and location information and what interactions do they infer? (ii) what relation information is mined?, (iii) what are the benefits of defining LLM workflows to mine large amounts of data?

==> sections/intro_v1.tex <==

Human population growth and expansion are coupled with the intentional and unintentional movement of species beyond their historic ranges. The introduction of nonnative species can have both direct and indirect impacts that cascade across ecological scales from individual plants and animals to populations and communities \cite{roy2023ipbes}. Examples of negative impacts due to the introduction and establishment of invasive species include but are not limited to competition for limited resources that impede native species growth and development, competitive exclusion and crashes of native populations, or disruptions to community ecology, such as impacts on food webs whereby reduction or removal of key species affect biological interactions up and down the trophic levels.  Invasion biology is defined as the study of species (populations and individuals) that have been redistributed outside their native geographic ranges as a result of human-mediated translocation \cite{cassey2018invasion}. The goal of invasion biology is to identify and understand the impacts of alien species on native flora and fauna across these ecological scales, not only to conserve rare, sensitive, and ecologically valuable native species, but also because intact functional ecosystems provide important economic, public health, and socioemotional services to humans \cite{jeschke2018invasion}. Despite the rapid rate and global scale of alien species introductions, a comprehensive categorization of these species and where they are located along with an understanding of their relationships with other species, is needed to assess current impacts on the ecosystems that they invade. Furthermore, understanding these basic relationships provides a first step toward predicting future invasions and consequences under scenarios of increasing human population growth and climate change.  

%from chapter: Invasion Biology: Searching for Predictions and Prevention, and Avoiding Lost Causes by Phillip Cassey et al.
%Alien species are also one of the major drivers of biodiversity loss worldwide. Invasive alien species have contributed to the extinction of more plants and animals since 1500 ad than any process other than habitat loss \cite{bellard2016alien}. 

%The ongoing establishment of new alien species, from almost all major taxa \cite{seebens2017no}, suggests that society is facing increasing economic and ecological costs from IAS in the coming decades \cite{essl2011socioeconomic}.

%The great variety of alien species, the widespread locations in which they have been released and become invasive pests, and the range of negative impacts arising from these pests has spawned a major research effort designed to understand (i.e. quantify and clarify) the invasion process, and provide the robust evidence-based activities needed to control and mitigate their impacts \cite{lockwood2013invasion}.

%why?
%why is it important to have structured summaries of insights from scientific papers
Given that we have a significant body of studies on different aspects of the invasion process, one good way to move forward is to interrogate this information attempting to identify consensus, or key aspects of variation, in our existing knowledge.

%how?
The nature of Information Extraction (IE) from scientific literature involves defining semantic schemas—structures specifying entities and their relationships—that together form a coherent unit of information. For example, the ``reproduction number ($R0$) estimates'' semantic model \cite{r0-estimate,shamsabadi-etal-2024-large} in virology defines core properties such as disease name, location, date, $R_0$ value, confidence interval (CI) values, and method, thereby producing a structured summary that showcases research contribution. Such structured summaries draw inspiration from Wikipedia infoboxes. Similarly, the Open Research Knowledge Graph (ORKG) \cite{auer2020improving} adopts this structured summary paradigm for representing scientific knowledge, enabling direct comparisons of similarly modeled research findings \cite{oelen2019comparing}. In essence, much like Amazon product comparisons, the ORKG’s structured summaries facilitate strategic reading practices by providing concise, easily interpretable overviews. This approach helps researchers navigate the increasingly growing body of scientific publications \cite{bornmann2021growth}, mitigating cognitive overload and fostering informed, efficient scholarship. 

The impetus behind this work lies in the push to transform unstructured scientific text into structured, machine-actionable insights. By doing so, researchers and practitioners can more easily perform precise queries, conduct automated comparisons, and integrate findings across different domains. This structured information enables advanced applications such as domain-specific knowledge discovery, automated literature reviews, improved evidence synthesis, intelligent recommender systems, cross-disciplinary data integration, and more efficient decision-support tools within the scientific enterprise. In the biomedical domain, NER and RE facilitate large-scale biomedical data analysis, such as network biology \cite{biomed1}, gene prioritization \cite{biomed2}, drug repositioning \cite{biomed3} and the creation of curated databases \cite{biomed4}. In the clinical domain, NER and RE can aid in disease and treatment prediction, readmission prediction, deidentification, and patient cohort identification \cite{miotto2018deep}. These advances present unexplored possibilities of exploration for ecology via ..


The scope of information extraction (IE) in this paper encompasses two key tasks: named entity recognition (NER), which involves extracting entities, and relation extraction (RE), which identifies relationships between entities. Traditional natural language processing (NLP) approaches to these tasks often rely on a pipeline structure, where NER is performed first, and its output is passed to the RE component \cite{luan2018multi}. However, this pipeline approach is prone to error propagation and prevents the two tasks from leveraging each other’s insights \cite{yan2022empirical}. Recent studies have shown that jointly learning NER and RE can mitigate error propagation and enhance overall performance \cite{giorgi2019end}. Building on this, advances in generative artificial intelligence—particularly large language models (LLMs)—open new opportunities for IE. A central question emerges: \textit{can LLMs, with their advanced pattern-recognition capabilities, be effectively applied to a new domain to simultaneously identify entities and infer their relationships?}

This work identifies the following four key entities in invasion biology--viz. species, location, habitat, and ecosystem. Automatically mining these entities and their relations from research papers present implications for various applications that can be built over such structured knowledge bases.

- Do the LLMs extract reasonable species and location information and what interactions do they infer?

- What relation information is mined?

- what are the benefits of defining LLM workflows to mine large amounts of data?
